Beyond Numbers: Creating Analogies to Enhance Data Comprehension and Communication with Generative AI

Unfamiliar measurements usually hinder readers from grasping the scale of the numerical data, understanding the content, and feeling engaged with the context. To enhance data comprehension and communication, we leverage analogies to bridge the gap between abstract data and familiar measurements. In this work, we first conduct semi-structured interviews with design experts to identify design problems and summarize design considerations. Then, we collect an analogy dataset of 138 cases from various online sources. Based on the collected dataset, we characterize a design space for creating data analogies. Next, we build a prototype system, AnalogyMate, that automatically suggests data analogies, their corresponding design solutions, and generated visual representations powered by generative AI. The study results show the usefulness of AnalogyMate in aiding the creation process of data analogies and the effectiveness of data analogy in enhancing data comprehension and communication.

==> figures/figures.tex <==
1.teaser (output)
2.data analogy example
3.dataset table/figure
4.design space (data analogy classification）
5.system interface
6.GPT chain of thought steps and results (ref:popblends) 
8.example questions (evaluation stimuli)
9.evaluation results


